Quantifying Emotional Responses to Immutable Data Characteristics and Designer Choices in Data Visualizations

Emotion is an important factor to consider when designing visualizations as it can impact the amount of trust viewers place in a visualization, how well they can retrieve information and understand the underlying data, and how much they engage with or connect to a visualization. We conducted five crowdsourced experiments to quantify the effects of color, chart type, data trend, data variability and data density on emotion (measured through self-reported arousal and valence). Results from our experiments show that there are multiple design elements which influence the emotion induced by a visualization and, more surprisingly, that certain data characteristics influence the emotion of viewers even when the data has no meaning. In light of these findings, we offer guidelines on how to use color, scale, and chart type to counterbalance and emphasize the emotional impact of immutable data characteristics.

==> instructions.tex <==
%% \section{Introduction} %for journal use above \firstsection{..} instead
This template is for papers of VGTC-sponsored conferences such as IEEE VIS, IEEE VR, and ISMAR which are published as special issues of TVCG.
The template does not contain the respective dates of the conference/journal issue, these will be entered by IEEE as part of the publication production process.
Therefore, \textbf{please leave the copyright statement at the bottom-left of this first page untouched}.


\section{Author Details}

You should specify ORCID IDs for each author (see \url{https://orcid.org/}  to register) for disambiguation and long-term contact preservation.
Use \verb|\authororcid{Author Name}{0000-0000-0000-0000}| for each author, replacing the ``Author Name'' and using the 16-digit (hyphenated) ORCID ID for the second parameter.
The template shows an example without ORCID IDs for two of the authors.
ORCID IDs should be provided in all cases.

Each author's affiliations have to be provided in the author footer on the bottom-left corner of the first page.
It is permitted to merge two or more people from the same institution as long as they are shown in the same order as in the overall author sequence on the top of the first page.
For example, if authors A, B, C, and D are from institutions 1, 2, 1, and 2, respectively, then it is ok to use 2 bullets as follows:
\begin{itemize}
  \item A and C are with Institution 1. E-mail: \{a\,$|$\,c\}@i1.com\,.

  \item B and D are with Institution 2. E-mail: \{b\,$|$\,d\}@i2.org\,.
\end{itemize}


\section{Hyperlinks and Cross References}

The style uses the \verb|hyperref| package which can typeset clickable hyperlinks using \verb|\href{...}{...}|, hyperlinked URLs using \verb|\url{...}|, and turns references into internal links.

The style also uses \verb|cleveref| to automatically and consistently format cross references.
We recommend that you use the \verb|\cref{label}| and \verb|\Cref{label}| calls instead of \verb|Figure~\ref{label}| or similar.
\verb|\Cref| should be used when starting a sentence to spell out the reference (e.g.\ ``Section'') while \verb|\cref| should be used when referencing within a sentence to abbreviate (e.g.\ ``Sec.'').
Here are examples for use within a sentence: \cref{fig:vis_papers}, \cref{tab:vis_papers}, \cref{sec:supplement_inst,sec:references_inst}, \cref{eq:sum}.
The following sentences all start with a reference, so use \verb|\Cref|.
\Cref{fig:vis_papers} is a \verb|figure| environment.
\Cref{tab:vis_papers} is a \verb|table| environment.
\Cref{sec:supplement_inst,sec:references_inst} are \verb|section| environments.
\Cref{eq:sum} is an \verb|equation| environment.


\section{Figures}

\subsection{Loading figures}

The style automatically looks for image files with the correct extension (eps for regular \LaTeX; pdf, png, and jpg for pdf\LaTeX), in a set of given subfolders defined above using \verb|\graphicspath|: figures/, pictures/, images/.
It is thus sufficient to use \verb|\includegraphics{CypressView}| (instead of \verb|\includegraphics{pictures/CypressView.jpg}|).
Figures should be in CMYK or Grey scale format, otherwise, colour shifting may occur during the printing process.

\subsection{Vector figures}

Vector graphics like svg, eps, pdf are best for charts and other figures with text or lines.
They will look much nicer and crisper and any text in them will be more selectable, searchable, and accessible.

\subsection{Raster figures}

Of the raster graphics formats, screenshots of user interfaces and text, as well as line art, are better shown with png.
jpg is better for photographs.
Make sure all raster graphics are captured in high enough resolution so they look crisp and scale well.

\subsection{Figures on the first page}

The teaser figure should only have the width of the abstract as the template enforces it.
The use of figures other than the optional teaser is not permitted on the first page.
Other figures should begin on the second page.
Papers submitted with figures other than the optional teaser on the first page will be refused.

\subsection{Subfigures}

You can add subfigures using the \texttt{subcaption} package that is automatically loaded.
Inside a \verb|figure| environment, create a \verb|subfigure| environment.
See \cref{fig:ex_subfigs} for an example.
You can reference individual figures, either fully using \verb|\cref| (\cref{fig:ex_subfigs_a,fig:ex_subfigs_b}) or by letter using \verb|\subref|.
E.g., \subref{fig:ex_subfigs_b}, \subref{fig:ex_subfigs_c}.
Note that \verb|\subref| only works for one label at a time.

\begin{figure}[tbp]
  \centering
  \begin{subfigure}[b]{0.45\columnwidth}
  	\centering
  	\includegraphics[width=\textwidth]{example-image-a}
  	\caption{The letter A.}
  	\label{fig:ex_subfigs_a}
  \end{subfigure}%
  \hfill%
  \begin{subfigure}[b]{0.45\columnwidth}
  	\centering
  	\includegraphics[width=\textwidth]{example-image-b}
  	\caption{The letter B.}
  	\label{fig:ex_subfigs_b}
  \end{subfigure}%
  \\%
  \begin{subfigure}[b]{0.45\columnwidth}
  	\centering
  	\includegraphics[width=\textwidth]{example-image-c}
  	\caption{The letter C.}
  	\label{fig:ex_subfigs_c}
  \end{subfigure}%
  \subfigsCaption{Example of adding subfigures with the \texttt{subcaption} package.}
  \label{fig:ex_subfigs}
\end{figure}

\subsection{Figure Credits}
\label{sec:figure_credits_inst}

In the \hyperref[sec:figure_credits]{Figure Credits} section at the end of the paper, you should credit the original sources of any figures that were reproduced or modified.
Include any license details necessary, as well as links to the original materials whenever possible.
For credits to figures from academic papers, include a citation that is listed in the \textbf{References} section.
An example is provided \hyperref[sec:figure_credits]{below}.


\section{Equations and Tables}

Equations can be added like so:

\begin{equation}
  \label{eq:sum}
  \sum_{j=1}^{z} j = \frac{z(z+1)}{2}
\end{equation}

Tables, such as \cref{tab:vis_papers} can also be included.


\begin{table}[tb]
  \caption{%
  	VIS/VisWeek accepted/presented papers: 1990--2016.%
  }
  \label{tab:vis_papers}
  \scriptsize%
  \centering%
  \begin{tabu}{%
  	  r%
  	  	*{7}{c}%
  	  	*{2}{r}%
  	}
  	\toprule
  	year & \rotatebox{90}{Vis/SciVis} &   \rotatebox{90}{SciVis conf} &   \rotatebox{90}{InfoVis} &   \rotatebox{90}{VAST} &   \rotatebox{90}{VAST conf} &   \rotatebox{90}{TVCG @ VIS} &   \rotatebox{90}{CG\&A @ VIS} &   \rotatebox{90}{VIS/VisWeek} \rotatebox{90}{incl.\ TVCG/CG\&A}   &   \rotatebox{90}{VIS/VisWeek} \rotatebox{90}{w/o TVCG/CG\&A}   \\
  	\midrule
  	2016 & 30 &   & 37 & 33 & 15 & 23 & 10 & 148 & 115 \\
  	2015 & 33 & 9 & 38 & 33 & 14 & 17 & 15 & 159 & 127 \\
  	2014 & 34 &   & 45 & 33 & 21 & 20 &    & 153 & 133 \\
  	2013 & 31 &   & 38 & 32 &    & 20 &    & 121 & 101 \\
  	2012 & 42 &   & 44 & 30 &    & 23 &    & 139 & 116 \\
  	2011 & 49 &   & 44 & 26 &    & 20 &    & 139 & 119 \\
  	2010 & 48 &   & 35 & 26 &    &    &    & 109 & 109 \\
  	2009 & 54 &   & 37 & 26 &    &    &    & 117 & 117 \\
  	2008 & 50 &   & 28 & 21 &    &    &    &  99 &  99 \\
  	2007 & 56 &   & 27 & 24 &    &    &    & 107 & 107 \\
  	2006 & 63 &   & 24 & 26 &    &    &    & 113 & 113 \\
  	2005 & 88 &   & 31 &    &    &    &    & 119 & 119 \\
  	2004 & 70 &   & 27 &    &    &    &    &  97 &  97 \\
  	2003 & 74 &   & 29 &    &    &    &    & 103 & 103 \\
  	2002 & 78 &   & 23 &    &    &    &    & 101 & 101 \\
  	2001 & 74 &   & 22 &    &    &    &    &  96 &  96 \\
  	2000 & 73 &   & 20 &    &    &    &    &  93 &  93 \\
  	1999 & 69 &   & 19 &    &    &    &    &  88 &  88 \\
  	1998 & 72 &   & 18 &    &    &    &    &  90 &  90 \\
  	1997 & 72 &   & 16 &    &    &    &    &  88 &  88 \\
  	1996 & 65 &   & 12 &    &    &    &    &  77 &  77 \\
  	1995 & 56 &   & 18 &    &    &    &    &  74 &  74 \\
  	1994 & 53 &   &    &    &    &    &    &  53 &  53 \\
  	1993 & 55 &   &    &    &    &    &    &  55 &  55 \\
  	1992 & 53 &   &    &    &    &    &    &  53 &  53 \\
  	1991 & 50 &   &    &    &    &    &    &  50 &  50 \\
  	1990 & 53 &   &    &    &    &    &    &  53 &  53 \\
  	\midrule               
  	\textbf{sum} & \textbf{1545} & \textbf{9} & \textbf{632} & \textbf{310} & \textbf{50} & \textbf{123} & \textbf{25} & \textbf{2694} & \textbf{2546} \\
  	\bottomrule
  \end{tabu}%
\end{table}

\begin{figure}[tb]% specify a combination of t, b, p, or h for top, bottom, on its own page, or here
  \centering % avoid the use of \begin{center}...\end{center} and use \centering instead (more compact)
  \includegraphics[width=\columnwidth]{paper-count-2016}
  \caption{%
  	A visualization of the 1990--2016 data from \cref{tab:vis_papers}, recreated based on Fig.\ 1 from \cite{Isenberg:2017:VMC}.%
  }
  \label{fig:vis_papers}
\end{figure}



\section{Supplemental Material Instructions}
\label{sec:supplement_inst}

In support of transparent research practices and long-term open science goals, you are encouraged to make your supplemental materials available on a publicly-accessible repository.
Please describe the available supplemental materials in the \hyperref[sec:supplemental_materials]{Supplemental Materials} section.
These details could include (1) what materials are available, (2) where they are hosted, and (3) any necessary omissions.


\section{References}
\label{sec:references_inst}

An example of the reference formatting is provided in the \textbf{References} section at the end.


\subsection{Include DOIs}

All references which have a DOI should have it included in the bib\TeX\ for the style to display.
The DOI can be entered with or without the \url{https://doi.org/} prefix.

\subsection{Narrow DOI option}

The \verb|-narrow| versions of the bibliography style use the font \verb|PTSansNarrow-TLF| for typesetting the DOIs in a compact way.
This font needs to be available on your \LaTeX\ system.
It is part of the \href{https://www.ctan.org/pkg/paratype}{\texttt{paratype} package}, and many distributions (such as MikTeX) have it automatically installed.
If you do not have this package yet and want to use a \verb|-narrow| bibliography style then use your \LaTeX\ system's package installer to add it.
If this is not possible you can also revert to the respective bibliography styles without the \verb|-narrow| in the file name.
DVI-based processes to compile the template apparently cannot handle the different font so, by default, the template file uses the \texttt{abbrv-doi} bibliography style.

\subsection{Disabling hyperlinks}

To avoid adding hyperlinks to the references (the default) you can use \verb|\bibliographystyle{abbrv-doi}| instead of \verb|\bibliographystyle{abbrv-doi-hyperref}|.
By default, the DOI field in a bib\TeX\ entry is turned into a hyperlink.

See the examples in the bib\TeX\ file and the bibliography at the end of this template.

\subsection{Guidelines for bibTeX}

\begin{itemize}
  \item All bibliographic entries should be sorted alphabetically by the last name of the first author.
        This \LaTeX/bib\TeX\ template takes care of this sorting automatically.
  \item Merge multiple references into one; e.\,g., use \cite{Max:1995:OMF,Kitware:2003} (not \cite{Kitware:2003}\cite{Max:1995:OMF}).
        Within each set of multiple references, the references should be sorted in ascending order.
        This \LaTeX/bib\TeX\ template takes care of both the merging and the sorting automatically.
  \item Verify all data obtained from digital libraries, even ACM's DL and IEEE Xplore  etc.\ are sometimes wrong or incomplete.
  \item Do not trust bibliographic data from other services such as Mendeley.com, Google Scholar, or similar; these are even more likely to be incorrect or incomplete.
  \item Articles in journal---items to include:
        \begin{itemize}
  	      \item author names
  	      \item title
  	      \item journal name
  	      \item year
  	      \item volume
  	      \item number
  	      \item month of publication as variable name (i.e., \{jan\} for January, etc.; month ranges using \{jan \#\{/\}\# feb\} or \{jan \#\{-{}-\}\# feb\})
        \end{itemize}
  \item Use journal names in proper style: correct: ``IEEE Transactions on Visualization and Computer Graphics'', incorrect: ``Visualization and Computer Graphics, IEEE Transactions on''
  \item Papers in proceedings---items to include:
        \begin{itemize}
  	      \item author names
  	      \item title
  	      \item abbreviated proceedings name: e.g., ``Proc.\textbackslash{} CONF\_ACRONYNM'' without the year; example: ``Proc.\textbackslash{} CHI'', ``Proc.\textbackslash{} 3DUI'', ``Proc.\textbackslash{} Eurographics'', ``Proc.\textbackslash{} EuroVis''
  	      \item year
  	      \item publisher
  	      \item town with country of publisher (the town can be abbreviated for well-known towns such as New York or Berlin)
        \end{itemize}

  \item Article/paper title convention: refrain from using curly brackets, except for acronyms/proper names/words following dashes/question marks etc.; example:\\\\
        %
        The paper ``Marching Cubes: A High Resolution 3D Surface Construction Algorithm'' should be entered as ``\{M\}arching \{C\}ubes: A High Resolution \{3D\} Surface Construction Algorithm'' or  ``\{M\}arching \{C\}ubes: A high resolution \{3D\} surface construction algorithm''.
        It will then be typeset as ``Marching Cubes: A high resolution 3D surface construction algorithm''
  \item For all entries:
        \begin{itemize}
  	      \item DOI can be entered in the DOI field as plain DOI number or as DOI url.
  	      \item Provide full page ranges AA-{}-BB
        \end{itemize}
  \item When citing references, do not use the reference as a sentence object; e.g., wrong: ``In \cite{Lorensen:1987:MCA} the authors describe \dots'', correct: ``Lorensen and Cline \cite{Lorensen:1987:MCA} describe \dots''
\end{itemize}

\section{Appendices}
\label{sec:appendices_inst}

Appendices can be specified using \verb|\appendix|.
For example, our Troubleshooting instructions in
\iflabelexists{appendix:troubleshooting}
  {\cref{appendix:troubleshooting}}
  {the appendix of the full paper at \url{https://osf.io/nrmyc}}.

Note that the paper submission has to end after the \textbf{References} section and within the page limit of the conference you are submitting to.
Any version of Appendices or the paper with Appendices included has to be submitted separately as supplementary material.
You can use the \verb|hideappendix| class option to remove everything after \verb|\appendix|.
We encourage you to submit a full version of your paper to a preprint server with any appendices included.

You can use the \verb|\iflabelexists| macro to cross reference an appendix from the main text, but only if that label (i.e.\ the appendix) actually exists.
For example, above we use 

\begin{verbatim}
\iflabelexists{appendix:troubleshooting}
  {\cref{appendix:troubleshooting}}
  {the appendix of the full paper at
   \url{https://osf.io/XXXXX}}.
\end{verbatim}

in order to cross-reference to the appendix with \verb|\cref| if it exists, but if the appendix is commented out then we will simply create a hyperlinked URL to it.


\section{Filler Text to Flush Out the Paper}

\lipsum[1-2]% Just add some more arbitrary text so we see a fuller paper example
